Knowledge-Grounded Self-Rationalization via Extractive and Natural Language Explanations

Models that generate extractive rationales (i.e., subsets of features) or natural language explanations (NLEs) for their predictions are important for explainable AI. While an extractive rationale provides a quick view of the features most responsible for a prediction, an NLE allows for a comprehensive description of the decision-making process behind a prediction. However, current models that generate the best extractive rationales or NLEs often fall behind the state-of-the-art (SOTA) in terms of task performance. In this work, we bridge this gap by introducing RExC, a self-rationalizing framework that grounds its predictions and two complementary types of explanations (NLEs and extractive rationales) in background knowledge. Our framework improves over previous methods by: (i) reaching SOTA task performance while also providing explanations, (ii) providing two types of explanations, while existing models usually provide only one type, and (iii) beating by a large margin the previous SOTA in terms of quality of both types of explanations. Furthermore, a perturbation analysis in RExC shows a high degree of association between explanations and predictions, a necessary property of faithful explanations.

==> files/table.tex <==
\begin{table*}[t!]
% \footnotesize
\begin{subtable}[t]{\textwidth}
% \centering
\resizebox{\textwidth}{!}{%
\centering
\begin{NiceTabular}{lccccccccccccccccccccc}
\toprule
& \multicolumn{7}{c}{\bf ComVE} & \multicolumn{7}{c}{\bf e-SNLI} & \multicolumn{7}{c}{\bf COSe}\\
\cmidrule(l{2pt}r{2pt}){2-8} \cmidrule(l{2pt}r{2pt}){9-15} \cmidrule(l{2pt}r{2pt}){16-22}
\bf Model  & \bf \!\!\!Acc.\!\!\! & \bf \!\!\!MET.\!\!\! & \bf \!\!BRTSc.\!\! & \bf \!\!\!BLRT.\!\!\! & \bf e-ViL\!\!\! & \bf Yes & \bf No & \bf \!\!\!Acc.\!\!\! & \bf \!\!\!MET.\!\!\! & \bf \!\!BRTSc.\!\! & \bf \!\!\!BLRT.\!\!\! & \bf e-ViL\!\!\! & \bf Yes & \bf No & \bf \!\!\!Acc.\!\!\! & \bf \!\!\!MET.\!\!\! & \bf \!\!BRTSc.\!\! & \bf \!\!\!BLRT.\!\!\! & \bf e-ViL\!\!\! & \bf Yes & \bf No\\
\midrule
Gold & 100 & -- & -- & -- & 91.6 & 79.3 & 1.1 & 100 & -- & -- & -- & 98.1 & 94.1 & 2.7 & 100 & -- & -- & -- & 84.8 & 74.5 & 1.8 \\
Task SOTA & 97.0 & -- & -- & -- & -- & -- & -- & \bf 93.1 & -- & -- & -- & -- & -- & -- & \bf 83.7 & -- & -- & -- & -- & -- & -- \\\midrule
% Neg-Heu & -- & 1.2 & 78.2 & 21.4 & 77.5 & 47.7 & 1.4 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
NILE 
% \cite{DBLP:conf/acl/KumarT20} 
& -- & -- & -- & -- & -- & -- & -- & 91.9 & 11.3 & 75.3 & 41.2 & 84.3 & 80.1 & 9.4 & -- & -- & -- & -- & -- & -- & -- \\
CAGE 
% \cite{DBLP:conf/acl/RajaniMXS19}  
& -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & 72.1 & 1.3 & 43.1 & 16.9 & 59.5 & 35.4 & 16.7 \\
WT5 
% \cite{DBLP:journals/corr/abs-2004-14546}  
& 96.1 & 3.4 & 86.4 & 27.0 & 67.7 & 46.2 & 11.0  & 92.1 & 12.3 & 75.3 & 42.3 & 85.3 & 82.7 & 12.8 & 81.0 & 2.2 & 52.0 & 22.4 & 73.0 & 53.9 & 10.5 \\
\midrule
\rowcolor{Gray}
%\rowcolor[gray]{.9}
% Mod-\ours{}
%   &  7.2 & 88.6 & 30.1 & 51.2 &  10.5 & 14.4 &  78.9 &  47.2 &  87.8 & 6.6 & 2.2 & 52.4 & 26.4 & 62.6 &  5.7 \\
\rowcolor{Gray}\ours{}-ZS  & 96.6 &  7.8 &  72.4 &  24.1 & 65.7 &  56.3 &  16.1 & 92.6 & 11.9 &  63.4 &  40.7 & 88.1 & 85.6 &  5.7 & 83.1 &  2.4 & 38.4 &  17.4 & 83.2 & 73.2 &  5.6 \\\midrule
\rowcolor{Gray}\ours{}  & \bf \underline{97.1} &  \bf 14.1 &  \bf 91.9 &  \bf 33.5 & 87.2 &  \bf 72.6 &  2.7 & \underline{92.9} & \bf 19.5 & \bf 86.6 &  \bf 51.4 & \bf 94.8 & \bf 93.8 &  3.7 &  \underline{83.5} & \bf 7.1 & \bf 60.4 &  \bf 30.5 & \bf 87.3 & \bf 74.4 &  2.1 \\
\rowcolor{Gray}\ours{}+  & \bf \underline{97.1} &  -- &  -- &  -- &  \bf 88.3 & \bf 72.5 &  \bf 1.1 & \underline{92.9} & -- &  -- &  -- &  \bf 95.4 & \bf 94.1 &  \bf 2.7 & \underline{83.5} & -- &  -- &  -- & \bf 87.8 & \bf 74.5 & \bf 1.8 \\
\rowcolor{Gray}\ours{}-NP 
% \cite{DBLP:conf/nips/LewisPPPKGKLYR020} 
& 96.5& 3.2 & 89.4 & 26.0 & 62.1 & 43.2 & 15.0 & 92.6 & 13.1 & 77.4 & 45.3 & 87.6 & 81.3 & 13.4 & 82.1 & 3.6 & 55.4 & 23.7 & 79.2 & 63.1 & 9.5 \\
\rowcolor{Gray}w/o KN Sel.  & 97.0 &  11.4 &  90.1 & 33.2 & 84.3 &  65.3 &  5.1 & 92.7 & 17.9 &  83.4 & 51.0 & 92.8 & 91.6 &  5.8 & 83.2 & 6.4 & 58.4 &  27.8 & 85.0 & 70.2 &  2.5 \\
\rowcolor{Gray}w/o KN \& ER
% \cite{DBLP:conf/acl/LewisLGGMLSZ20} 
& 96.1 & 4.4 & 85.2 & 26.2 & 66.5  & 41.2 &7.6 & 92.2 & 12.3 & 76.4 & 41.8 & 82.8 &  81.2 & 15.6 & 80.8 & 2.4 & 51.6 & 22.3 & 65.9 & 44.0 & 15.8 \\
\bottomrule
% \midrule
\end{NiceTabular}%
}
% \vspace{-1ex}
\caption{}
% \caption{\small \textbf{Task performance (Acc.) and NLE quality for the NL tasks.} Automatic metrics: METEOR (MET.), BERTScore (BRTSc.), BLEURT (BLRT.), and human evaluation metrics: e-ViL score, Yes/No \%s. \textbf{Bold} indicates best numbers
% % significant differences
% ($p < 0.05$). \underline{Underline} indicates SOTA task performance from a model with explanations.
% }
% \label{tab:nl}
\end{subtable}%
\\
\bigskip
\begin{subtable}[t]{\textwidth}
\centering
% \centering
\resizebox{0.80\textwidth}{!}{%
\centering
\begin{tabular}{lcccccccccccccc}
\toprule
& \multicolumn{7}{c}{\bf e-SNLI-VE} & \multicolumn{7}{c}{\bf VCR}\\
\cmidrule(l{2pt}r{2pt}){2-8} \cmidrule(l{2pt}r{2pt}){9-15}
\bf Model  & \bf Acc. & \bf MET. & \bf BRTSc. & \bf BLRT. & \bf e-ViL & \bf Yes & \bf No & \bf Acc. & \bf MET. & \bf BRTSc. & \bf BLRT. & \bf e-ViL & \bf Yes & \bf No\\
\midrule
% & \bf System $\rightarrow$  & \bf Gold & \bf ROUGE & \bf BERTSc. & \bf METEOR & \bf SPICE  & \bf CIDEr & \bf BLEURT & \bf Yes & \bf W-Yes & \bf W-No & \bf No\\
Gold & 100 & -- & -- & -- & 90.6 & 79.3 & 1.1 & 100 & -- & -- & -- & 95.8 & 94.1 & 2.7\\
Task SOTA & 79.5 & -- & -- & -- & -- & -- & -- & 81.6 & -- & -- & -- & -- & -- & --  \\\midrule
PJ-X 
% \cite{DBLP:conf/cvpr/ParkHARSDR18}
& 69.2 & 14.7 & 79.1 & 35.6 & 70.1 & 55.2 & 14.5 & 39.0 & 16.4 & 78.4 & 43.5 & 73.9 & 58.2 & 10.5 \\
FME
% \cite{DBLP:journals/corr/abs-1809-02805}
& 73.7 & 15.6 & 79.7 & 34.5 & 71.9 & 56.7 & 13.2 & 48.9 & 17.3 & 79.4 & 47.8 & 73.0 &  56.2 & 11.1 \\
RVT
% \cite{DBLP:conf/emnlp/MarasovicBPBSC20}
& 72.0 & 18.8 & 81.1 & 35.3 & 72.2 & 55.4 & 12.8 & 59.0 & 11.2 & 78.9 & 44.2 & 73.2 & 57.4 & 11.5 \\
e-UG
% \cite{DBLP:journals/corr/abs-2004-14546}
& 79.5 & 19.6 & 81.7 & 37.8 & 75.6 & 57.9 & 9.9 & 69.8 & 11.8 & 79.0 & 45.6 & 75.1 & 59.3 & 10.4 \\
\midrule
% \rowcolor{Gray}Mod-\ours{}  &  21.4 & 85.6 & 39.2 & 60.4 & 8.3 & 18.9 & 83.6 & 50.2 & 65.3 & 9.3 \\
\rowcolor{Gray}\ours{}-ZS  &  78.6 & 12.4 &  78.7 & 35.9 &  79.7 & 60.7 & 10.3 & 79.2 & 15.7  & 78.9 & 41.4 & 78.9 & 65.2 &  10.2 \\ \midrule
\rowcolor{Gray}\ours{}  & \bf 80.8 & \bf 22.9 &  \bf 87.5 &  \bf 39.6 & \bf 81.6 & 64.2 & \bf 6.4 & \bf 79.5 & \bf 20.8 &  \bf 86.5 &  \bf 53.2 & 80.9 & \textbf{67.7} &  7.3   \\
\rowcolor{Gray}\ours{}+  & \bf 80.8 &  -- &  -- &  -- &  \bf 82.0 & \bf 65.3 &  \bf 6.3 & \bf 79.5 & -- &  -- &  -- & \bf 81.7 & 67.0 &  \bf 6.3 \\
\rowcolor{Gray}\ours{}-NP
% \cite{DBLP:conf/nips/LewisPPPKGKLYR020}
& 78.9 & 20.6 & 83.4 & 38.2 & 78.3 & 59.3 & 10.2 & 78.9 & 14.5 & 81.3 & 47.2 & 78.3 & 62.1 & 11.2 \\
\rowcolor{Gray}w/o KN Sel.  & 79.3 &  22.4 &  86.7 & \bf 39.6 &  79.8 & 62.3 & 7.9 & 78.6 & 19.7 & 85.4 & 51.3 & 79.9 & 67.2 &  8.2 \\
\rowcolor{Gray}w/o KN \& ER
% \cite{DBLP:journals/corr/abs-2004-14546}
& 79.5 & 19.6 & 81.7 & 37.8 & 75.6 & 57.9 & 9.9 & 69.8 & 11.8 & 79.0 & 45.6 & 75.1 & 59.3 & 10.4 \\
\bottomrule
\end{tabular}%
}
\caption{}
% \vspace{-1ex}
% \caption{\small \textbf{Task performance (Acc.) and NLE quality for the VL tasks.} Automatic metrics: METEOR (MET.), BERTScore (BRTSc.), BLEURT (BLRT.), and human evaluation metrics: e-ViL score, Yes/No \%s. \textbf{Bold} denotes significant differences ($p < 0.05$). \ours{}+ adds the selected knowledge with the generated NLEs, hence is only used in the human evaluations.
% }
% \label{tab:vl}
% \vspace{-1em}
\end{subtable}
\caption{\small \textbf{Task performance (Acc.) and NLE quality for the VL tasks.} Automatic metrics: METEOR (MET.), BERTScore (BRTSc.), BLEURT (BLRT.), and human evaluation metrics: e-ViL score, Yes/No \%s. \textbf{Bold} denotes significant differences ($p < 0.05$). \ours{}+ adds the selected knowledge with the generated NLEs, hence is only used in the human evaluations.}
\end{table*}
